PhyScene: Physically Interactable 3D Scene Synthesis for Embodied AI

With recent developments in Embodied Artificial Intelligence (EAI) research, there has been a growing demand for high-quality, large-scale interactive scene generation. While prior methods in scene synthesis have prioritized the naturalness and realism of the generated scenes, the physical plausibility and interactivity of scenes have been largely left unexplored. To address this disparity, we introduce PhyScene, a novel method dedicated to generating interactive 3D scenes characterized by realistic layouts, articulated objects, and rich physical interactivity tailored for embodied agents. Based on a conditional diffusion model for capturing scene layouts, we devise novel physics- and interactivity-based guidance mechanisms that integrate constraints from object collision, room layout, and object reachability. Through extensive experiments, we demonstrate that PhyScene effectively leverages these guidance functions for physically interactable scene synthesis, outperforming existing state-of-the-art scene synthesis methods by a large margin. Our findings suggest that the scenes generated by PhyScene hold considerable potential for facilitating diverse skill acquisition among agents within interactive environments, thereby catalyzing further advancements in embodied AI research. Project website: http://physcene.github.io.

==> sec/3_preliminarties.tex <==
\section{Preliminaries}\label{sec:prelim}

\begin{figure}[t!]
\centering
\fbox{\rule[0cm]{0cm}{5cm}\rule[0cm]{\linewidth}{0cm}}
\caption{\textbf{Model architecture of the \textsc{physcene}}. We use xxx. The xxx, xxx, and xxx optimizer serve as the guidance for physically-plausible and interactable scene synthesis.}
\label{fig:structure}
\end{figure}

==> tex/config_save.tex <==
% Common packages
\usepackage{graphicx}
\usepackage{times}
\usepackage{comment}
\usepackage{amsmath,amssymb,amsfonts,mathabx,mathbbol}
\usepackage{acronym}
\usepackage{enumitem}
% \usepackage[dvipsnames]{xcolor}
\PassOptionsToPackage{dvipsnames,table}{xcolor}
% \definecolor{uclablue}{rgb}{0.2,0.55,0.8}
% \usepackage[pagebackref,colorlinks,breaklinks,citecolor=uclablue]{hyperref}
\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,colorlinks,breaklinks,citecolor=cvprblue]{hyperref}
\usepackage{url}
\usepackage{balance}
\usepackage{xspace}
\usepackage{setspace}
\usepackage[skip=3pt,font=small]{subcaption}
\usepackage[skip=3pt,font=small]{caption}
\usepackage{caption}
\usepackage[misc]{ifsym}
\usepackage[capitalise]{cleveref}
\usepackage{tabularx}
\usepackage{multirow,multirow,array,makecell}
\usepackage{overpic}
\usepackage{wrapfig}
\usepackage{pifont}
\usepackage{url}
\usepackage{booktabs,tabularx,colortbl}         % professional-quality tables
\usepackage[utf8]{inputenc}                     % allow utf-8 input
\usepackage[T1]{fontenc}                        % use 8-bit T1 fonts
\usepackage{nicefrac}                           % compact symbols for 1/2, etc.
\usepackage[nopatch=footnote]{microtype}        % microtypography
\usepackage[noend,ruled,vlined]{algorithm2e}
\usepackage{algorithmic}
\usepackage{rotating}
\usepackage{adjustbox}
\usepackage{hvfloat}

% Handy shorthand
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} 
\def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother
\newcommand{\sota}{\text{state-of-the-art}\xspace}
\newcommand\supp{\textit{supplementary}\xspace}

% Handy math ops, more in math_commands.tex
\DeclareMathOperator{\ELBO}{\mathrm{ELBO}}
\DeclareMathOperator{\HH}{\mathcal{H}}
\DeclareMathOperator{\II}{\mathcal{I}}
\DeclareMathOperator{\LL}{\mathcal{L}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\N}{\mathcal{N}}

\newcommand{\dec}[1]{\textcolor{blue}{#1}}
\newcommand{\inc}[1]{\textcolor{red}{#1}}

% Special Characters
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

% Comments
\newcommand{\bx}[1]{\textcolor{red}{[BX: #1]}\xspace}
\newcommand{\sy}[1]{\textcolor{blue}{[SH: {#1}]}\xspace}

% Spacing
% \frenchspacing
% \medmuskip=2mu   % reduce spacing around binary operators
% \thickmuskip=3mu % reduce spacing around relational operators
% \setlength{\abovedisplayskip}{6pt}
% \setlength{\belowdisplayskip}{6pt}
% \setlength\abovecaptionskip{3pt}
% \setlength\belowcaptionskip{0pt}
% \setlength\floatsep{0.2\baselineskip plus 3pt minus 2pt}
% \setlength\textfloatsep{0.2\baselineskip plus 3pt minus 2pt}
% \setlength\dbltextfloatsep{0.2\baselineskip plus 3pt minus 2 pt}
% \setlength\intextsep{0.2\baselineskip plus 3pt minus 2 pt}

\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0ex \@plus 0ex \@minus 0ex}{-1em}%
  {\hskip\parindent\normalfont\normalsize\bfseries}%
}
\makeatother

% Clever references
\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Fig.}
\Crefname{figure}{Figure}{Figure}

% Graphics path
\graphicspath{{figures/}}

% Acronym, tasks
\acrodef{nlp}[NLP]{Natural Language Processing}
\acrodef{vos}[VOS]{Video Object Segmentation}

% Acronym & Short-hands, modules
\acrodef{gru}[GRU]{Gated Recurrent Unit}
\acrodef{mhsa}[MHSA]{Multi-Head Self-Attention}
\acrodef{mha}[MHA]{Multi-Head Attention}
\newcommand{\sa}{\text{Slot-Attention}\xspace}
\newcommand{\lnorm}[1]{\text{LayerNorm}({#1})\xspace}
\newcommand{\attn}[1]{\text{Attn}({#1})\xspace}
\newcommand{\ffn}[1]{\text{FFN}({#1})\xspace}

% Acronym, metrics
\acrodef{ari}[ARI]{Adjusted Rand Index}
\acrodef{msc}[MSC]{Mean Segmentation Covering}
\acrodef{miou}[mIoU]{mean Intersection over Union}
\acrodef{mse}[MSE]{Mean Squared Error}

% Acronym, Institution
\acrodef{ucla}[UCLA]{University of California, Los Angeles}
\acrodef{pku}[PKU]{Peking University}
\acrodef{thu}[THU]{Tsinghua University}
\acrodef{bigai}[BIGAI]{Beijing Institute for General Artificial Intelligence}

% Helper meta-texts
\newcommand{\model}{SceneDiffuser$^{++}$\xspace}


% Table
\definecolor{scope}{RGB}{103,78,167}
\definecolor{semantic}{RGB}{230,145,56}
\definecolor{type}{RGB}{153,0,0}
\definecolor{revision}{RGB}{0,0,0}

% thanks symbol
\makeatletter
\renewcommand*{\@fnsymbol}[1]{\ensuremath{\ifcase#1\or *\or \dagger\or \ddagger\or
   \mathsection\or \mathparagraph\or \|\or **\or \dagger\dagger
   \or \ddagger\ddagger \else\@ctrerr\fi}}
\makeatother
